Quality of Consumption: The Friendlier Side of Quality of Service

Cloud services today are increasingly built using functionality from other running services. In this paper, we question whether legacy Quality of Services (QoS) metrics and enforcement techniques are sufficient as they are producer centric. We argue that, similar to customer rating systems found in banking systems and many sharing economy apps (e.g., Uber and Airbnb), Quality of Consumption (QoC) should be introduced to capture different metrics about service consumers. We show how the combination of QoS and QoC, dubbed QoX, can be used by consumers and providers to improve the security and management of their infrastructure. In addition, we demonstrate how sharing information among other consumers and providers increase the value of QoX. To address the main challenge with sharing information, namely sybil attacks and mis-information, we describe how we can leverage cloud providers as vouching authorities to ensure the integrity of information. We present initial results in prototyping the appropriate abstractions and interfaces in a cloud environment, focusing on the design impact on both service providers and consumers.

==> Makefile <==
BUILD_DIR = .
OUTPUTDIR_OPTION = --output-directory $(BUILD_DIR)
SRC_FILES = ibm.bib refs.bib hotnets15.tex \
			abstract.tex \
			intro.tex \
			defining-qox.tex \
			sharing.tex \
			challenges.tex \
			personalization.tex \
			eval.tex \
			related.tex \
			conclusion.tex 


FIGURES_DIR = figures

all: hotnets15.pdf

hotnets15.pdf: $(SRC_FILES) $(FIGURES_DIR) 
	@if [ ! -d "$(BUILD_DIR)" ]; then mkdir -p $(BUILD_DIR); fi
	@-pdflatex $(OUTPUTDIR_OPTION) hotnets15.tex
	@-bibtex $(BUILD_DIR)/hotnets15
	@pdflatex $(OUTPUTDIR_OPTION) hotnets15.tex
	@pdflatex $(OUTPUTDIR_OPTION) hotnets15.tex

.PHONY: clean
clean:
	@cd $(BUILD_DIR) && rm -f *.aux *.bbl *.blg *.dvi *.log *.pdf *.ps


==> challenges.tex <==
\section{Challenges}
\subsection{Defining quality/metrics}
\subsection{Mapping quality matrices to actions}
\nip{Interpretation of a Reputation.}  Depending on the service,
reputations can be interpreted in many ways. Here, there is challenge
in defining what constitutes good or bad, and doing it automatically
(\ie a human will not be explicitly marking something as good or bad).
Even more, in machine-to-machine communication, an interaction is not
necessarily binary (good or bad), as there is a wide range of possible
interactions.

\subsection{Integrating and implementing QoX to service provider and consumers' components.}
Cloud components and services come in all shapes and
sizes. Integrating a reputation-based system do not require
substantial development efforts. Similar to service life-cycle
calls in PaaS clouds~\cite{cloudfoundry}, a QoX system must define
simple, yet generic interfaces that can be easily implemented by
service providers. More importantly, the interfaces should support
configurable query language that provides support for efficient
continuous query and feedback.

We have built a prototype of the QoX system, and
integrated it with several cloud components as shown in table

\begin{table*}[t]
\small
\centering
\newcommand\T{\rule{0pt}{2.6ex}}
\newcommand\B{\rule[-1.2ex]{0pt}{0pt}}
\begin{tabular}{|m{1.2in}|m{1in}|m{4in}|}
%\begin{tabular}{|p{1.2in}|p{1in}|p{4in}|}
\hline
\rowcolor[gray]{0.9} {\bf Category} & {\bf System} &  {\bf Description} \T \B \\
\hline
IaaS SDN Controller & Floodlight~\cite{floodlight} & The shim maps the reputation to OpenFlow rules via the Floodlight REST API to block or direct traffic. \\
\hline
PaaS Broker & CloudFoundry~\cite{cloudfoundry} & The shim interfaces between the CloudFoundry broker and the CloudFoundry  command line interface (used by the users) to filter and sort the marketplace results based on their reputation. \\
\hline
Load Balancer & HAProxy~\cite{haproxy} & This shim alters the configurations written in a haproxy.cfg file to specify load balancing based on the reputation (directing tenants to servers based on reputation).  Upon every change, the shim will tell HAProxy to reload the configuration. \\
\hline
Infrastructure Monitoring & Nagios~\cite{nagios} & We took advantage of JNRPE (Java Nagios Remote Plugin Executor)~\cite{jnrpe} to build a Java plugin that is listening for any reputations sent by Seit's reputation manager, and displays this sentiment and configures alerts for when sentiment (collective reputation of the tenant running Nagios) drops. \\
\hline
Intrusion Detection System & Snort~\cite{snort} & Snort alerts are configured to log to Syslog.  By using SWATCH~\cite{swatch} to monitor Syslog, the Seit shim is alerted to all Snort alerts.  The shim parses the alerts and extracts information such as source IP and alert type and send the feedback to the reputation manager. \\
\hline
\end{tabular}
\vspace{-0.1in}
\caption{Implemented shims}
\label{tab:plugins}
\end{table*}

\subsection{Sharing information how and to who}
\subsubsection{How}
Challenges: there are no clear, standardized way to compare quantifiable metrics for 
different services.  Instead, we are inspired by review systems found in web sites such
as Yelp (for restaurants) and Amazon (for products).

% Note: ostra really had binary, wanted/unwanted

Our rating system will consist of:

* Scaled rating -- instead of just good/bad or wanted/unwanted, have a scaled rating to 
  reflect varying quality. 

* Coarse Sub-categories -- e.g., home depot has quality and value in addition to overall rating.
  

* Text based reviews -- in case a human reads, or find common comments (like Amazon does) 
  without having to standardize on specific event feedback tags.  Basically to tease out
	what criteria a given party used. (e.g., an ethnic restaurant that some complain isn't 
	authentic enough, so gave it 3 stars, when a diner might be fine with that as long as its
	tasty and clean) 

To achieve this, we need a system designed to tie events and monitoring frameworks to 
feedback that affect both the rating and the text.

\subsection{Preventing gaming aspect to the system}
\subsubsection{Cloud Provider as Vouching Authority}
Two key challenges arise when dealing with any sharing -- ensuring the validity 
of information.  As we move toward an entirely cloud based infrastructure, both IaaS 
and Paas, we believe we gain an opportunity to overcome these challenges.
In this section we address two main categories of information, and how the cloud
provider can play a role to reduce the ability to lie. 


\subsubsection{Real-time, Actionable Information}	

Some information would cause immediate, automated action and as such lying can
have a negative impact.  Consider one service provider detecting the start of some
attack (e.g., a DoS attack) -- sharing this information with another provider will
help them, say block that user, but if they are able to lie about it, they can cause
another service provider to block a user unnecessarily.  So, we need to ensure the
information is accurate.

System of records

Provider as a certifying authority that some specific event occurred.
Here, the tenant can specify certain things that the cloud provider can
vouch happened.

Bursts of traffic, crashes, that a specific IP address did indeed send something to 
another IP address.

if PaaS provider, maybe more.

\subsection{Evaluating the system}

==> eval.tex <==
\section{Initial Results}

Perhaps part prototype, part eval.

Things we might evaluate:

Integration

Benefits of QoC

The practicality of our claim of vouching

==> motivation.tex <==
\section{The need for service consumer quality and engagement}
In many successful business models, it became a necessary for a service provider to select and grade his costumers based on some matrices the provider defines. This selection eventually provides an impact on the service’s provider business and revenue. This model is followed by many law firms, manufactures, financial companies, and even restaurants and hotels. The quality and care given to certain type of customers do not necessary mean that this costumer will pay a higher amount. Instead, it can potentially leads to more connections and longer business. 
To make a simple example, a landlord can set certain criteria for his prospective tenants (large deposit, strong recommendation letter from previous landlord, minimum age, etc.). This criteria will lead potential better tenants (more responsible, less partying and bothering other tenants) which also leads to a better rate for the building/neighbor and its landlord. At the same time, landlord may take actions to certain behaviors by tenants (annoying neighbors or damaging the property) such as warranty letter or canceling the leasing contract. 

We believe that business model between service providers and consumers in the cloud can be framed as the above mentioned models. In addition, service providers can share feedback of their consumers to detect misbehaving consumers and apply security configuration a head of time. At the same time, service consumer can share their relation experience with service provider in order to rate their services, leading to an environment where services are forced to enhanced their application or run out of business.  
In this section, we elaborate on the potential benefits provided by a system that leverages the engagement between service providers and consumers. Exploring different examples, we then
identify the key design challenges in building such system.

\subsection{From Service Provider Perspective}
\nip{The ability to classify consumers}
A reputation-based system for service consumers can be useful for service providers during  and after the binding phase, since it maintains historical information on consumers of the service. In CloudFoundry, for example, the service provider
(\eg ClearDB and MongolabDB) is responsible to implementing multi-tenancy. Most data stores do not create separate containers (or VMs) per tenant; they
simply create different table spaces for each tenant. With a reputation-based system,
service providers can implement different tenant isolation
primitives. An untrusted user is provisioned a separate container
and is charged more because of the additional computing resources that
are required.
In addition, there is big overload on resources used by service providers to monitor and and analyse their consumer traffic (e.g. IDS and Firewall). By classifying consumers to catogroes based on their securoty level, resources can be optimized by focusing on high security threat consumers. 

\nip{Encourage a culture of self-policing}
In traditional 
infrastructures, the administrator has great
visibility of what is happening inside of the infrastructure through a
variety of monitoring tools.  The administrator, however, has limited
visibility into how the infrastructure is viewed externally.  
Major outages are obvious and are easy to detect. Other
types of issues might, at best, result in an email (or other reporting
mechanism) being sent to the administrator.  
Sentiment analysis is widely used in corporations (\eg monitor Twitter feeds
to observe whether there is any positive or negative chatter affecting
its brand~\cite{henshen2012, o2010tweets}).  With a reputation-based system,
a service can monitor its sentiment as perceived by its consumers.  By
monitoring one's sentiment, the tenant can determine whether others
are having a negative experience interacting with it, then trigger a
root cause analysis.  This is supported by a report from
Verizon~\cite{verizon} which says that in many cases, infiltrations
are largely detected by external parties, not by the infected party
itself.

\nip{Signifitley reduce the need for manual/static configuration}
A major limitation in services now days is the static configuration and the difficulty to meet the dynamic environment of the cloud. For example, services that provide storage or web access to multiple servers use loadbalancers to load and spread the traffic among servers. By receiving automated updaes about consumers' reputations, this info can be mapped to loadbalancer configurations to redirect traffic of certain consumers.
Figure~\ref{fig:ex_tenant} illustrates the integration of a reputation-based system into a
web service, where load balancers are used to distribute
client load across identical instances of the service.  Typically,
load balancers aim for even distribution~\cite{nginx}. 
%(while, of course, supporting
%sticky sessions to ensure subsequent requests from the same client go
%to the same server)~\cite{nginx}.
With a reputation-based system, the web service can differentiate its users based on their
reputation, directing good/trusted clients to a set of
servers, and bad/untrusted clients to a different set of servers.
\begin{figure}[t]
\centering
\includegraphics[width=0.8\columnwidth]{figures/motivation_ex_tenant.pdf}
\caption{Example of a tenant using a reputation-based system}
\label{fig:ex_tenant}
\vspace{-0.1in}
\end{figure}   

\subsection{From Service Consumer Perspective}
\nip{The ability to rate service providers}
Surprisingly, cloud service marketplaces such as Heruko, Pivtol, and Mashup, lack any rating for the services they provide to their platform users. Leaving the user to only try, and in many cases, pay for the service before deciding if this service meets the his requirements in terms of quality and efficiency.
Providing a rating system to service users not only enhance their experience and choice to choose services but also put the pressure on service provider to enhance their services to receive better rating, and encourage the culture of self-policing as mentioned above.

PaaS clouds offer the ability
to compose applications using services provided by the platform.  In
some cases, a PaaS cloud provides all of the services (\eg
Microsoft Azure~\cite{windowsazure}).  In other cases, platforms, such as
CloudFoundry~\cite{cloudfoundry}, provide an environment where many
service providers can offer their services.

As illustrated in Figure~\ref{fig:ex_paas}, service consumers use a
{\em broker} to (1) discover services and (2) bind to them. Service
discovery, in general, implements a simple search capability, focusing
on returning one-to-one match with the needed service (\eg version 2.6
of MongoDB).  With a reputation-based system, service discovery can be
enriched to include many new metrics that capture the quality of
service as perceived by other users. So, if two different providers
offer version 2.6 of MongoDB, then consumers can reason about which
service offer better quality.

\begin{figure}
\centering
\includegraphics[width=0.9\columnwidth]{figures/motivation_ex_paas.pdf}
\caption{Example of a PaaS provider using a reputation-based system}
\label{fig:ex_paas}
\vspace{-0.1in}
\end{figure}

\nip{Encourage a culture of more efficient, stable, and reliable consumers}
Wordpress example

\subsection{Challenges}
\label{sec:challenges}

Applying to the cloud has the unique challenges in being machine-to-machine,
highly variable, and highly dynamic interactions. In this subsection, we identify challenges when building a cloud-based reputation-based
system.
\nip{Defining quality/metrics.}

\nip{Integration.} Cloud components and services come in all shapes and
sizes. Integrating a reputation-based system do not require
substantial development efforts. Similar to service life-cycle
calls in PaaS clouds~\cite{cloudfoundry}, a reputation-based system must define
simple, yet generic interfaces that can be easily implemented by
service providers. More importantly, the interfaces should support
configurable query language that provides support for efficient
continuous query and feedback.

\nip{Interpretation of a Reputation.}  Depending on the service,
reputations can be interpreted in many ways. Here, there is challenge
in defining what constitutes good or bad, and doing it automatically
(\ie a human will not be explicitly marking something as good or bad).
Even more, in machine-to-machine communication, an interaction is not
necessarily binary (good or bad), as there is a wide range of possible
interactions.


\nip{Mapping quality matrices to actions.}
\nip{Sharing information how and with who}
\nip{Preventing gaming aspect to the system.}
\subsubsection{Raising reputation/rate to gain security access then attack.}
\nip{Evaluating the system.}

